Min-cuts and Shortest Cycles in Planar Graphs in O(n log log n) Time

We present a deterministic O(n log log n) time algorithm for finding shortest cycles and minimum cuts in planar graphs. The algorithm improves the previously known fastest algorithm by Italiano et al. in STOC'11 by a factor of log n. This speedup is obtained through the use of dense distance graphs combined with a divide-and-conquer approach.

==> holes-bak.tex <==
\section{Dealing with holes}

In this section we show how to deal with some issues that might arise when the $r$-division contains holes.
By Theorem \ref{theorem-r-division}, we can assume that there are is at most a constant number of holes in every piece.

\subsection{Intersecting pieces with a cycle}
In the dividing step of the algorithm we intersect some pieces with the interior and exterior of a cycle $C_e$.
This is done implicitly, by inserting division edges, but if a piece has holes, the embedding of the edge be homotopic to its corresponding path. 

This cycle $C_e$ consists of edges from dense distance graphs and a path going within one piece.
We cut this piece by tracking the cycle and rebuilding dense distance graphs on its both sides in $O(r \log r)$ time.
It remains to describe how to intersect a piece $P$ with a cycle consisting of edges from the dense distance graph.

We consider the subgraph of the skeleton graph induced by border vertices of $P$.
It has one connected component that is composed of border vertices that do not belong to any hole.
Let us call this component a \emph{frame} of $P$.

We take a subpath of $C_e$ that connects two vertices of frame of $P$ (call this subpath $C_P$).
$C_e$ can go through $P$ multiple times, but we consider all such subpaths one at a time.

First, we cut all holes recursively, so we can replace every part of $C_P$, which is contained within one hole, with a single edge.
$C_P$ cuts this graph into two parts.
For each hole we need to compute which part it belongs to.
This is easy if a hole is cut into two pieces with $C_P$, but a bit more complex in other cases.

We extend the initial computation of the dense distance graph.
Assume that there are $l$ holes $H_1, H_2, \cdots, H_l$.

We add a dummy border vertex $s$ to the frame of $P$ and connect it with an edge to a non-border vertex in $P$.
The edge length should be big, so that no shortest path between border vertices would go through $s$.
It suffices if its bigger than the sum of all edge lengths in $P$.

Now for each hole we fix some border vertex $b_i$, find the shortest path $K_i$ from $s$ to $b_i$ and make an incision along it.
For each vertex $v$ on the path, we obtain its two copies $v'$ and $v''$, which we connect with an edge of zero length.
Denote the set of those edges by $E_i$.

After that, for each edge of the dense distance graph we want to compute whether its underlying shortest path contains any edges from any of $E_i$.
In order to do that, we modify edge lengths.
We use $l+2$ tuples to measure lengths of paths.
The first element of the tuple is the sum of original edge lengths.
The second element is the number of edges from \emph{any} $E_i$.
The $j+2$-th element is the number of edges from $E_j$.
Hence, the second element is the sum of the elements following it.

The tuples are compared in lexicographic order, which assures that the shortest paths are not affected with this operation.
Nor is the running time, as there is a constant number of holes.
As every $K_i$ is a shortest path and we minimize the number of times we cross any $K_i$, any shortest path would contain at most one element from each $E_i$.

The modified distances allow us to determine, which side of $C_P$ does every hole lie on.
If some path does not contain any edges from $E_i$, then $H_i$ is on the same side of $C_P$ as $s$.
Otherwise, $H_i$ and $s$ are on different sides of $C_P$.

Lastly, we have to cut the dense distance graph of $P$ into two parts.
We simply insert one division edge to the recursion graph and assume that the distances inside each part are equal to distances inside $P$.
This is in general incorrect for pieces with holes, as some shortest path might cross $C_P$ many times.
Hence, it might occur that the real distance between two vertices is bigger than we have assumed.
This, however, does not affect our final result, as every distance corresponds to some valid path in the original graph, contained within the same piece.

The lengths of the edges are used only in minimum $st$-separating cycle computation in the conquering step ($s$ and $t$ are faces), carried out with Italiano \emph{et al.} algorithm~\cite{italiano-11}.
If we take the computed cycle and map every edge of the dense distance graph to the shortest path, which determines the length of this edge, we obtain a closed walk.
We have to show that this walk bounds some nonempty set of faces in the graph.
This follows easily from the algorithm, as it works with a graph composed of pieces containing $s$ and $t$ and dense distance graphs of all other pieces.
As a result, we obtain a closed walk, which has nonempty interior.
It can be shorter than the shortest cycle contained within the currently considered part of the graph, but is surely not shorter than the globally shortest cycle.

